A Comprehensive Survey on Graph Anomaly Detection with Deep Learning

Anomalies represent rare observations (e.g., data records or events) that deviate significantly from others. Over several decades, research on anomaly mining has received increasing interests due to the implications of these occurrences in a wide range of disciplines. Anomaly detection, which aims to identify rare observations, is among the most vital tasks in the world, and has shown its power in preventing detrimental events, such as financial fraud, network intrusion, and social spam. The detection task is typically solved by identifying outlying data points in the feature space and inherently overlooks the relational information in real-world data. Graphs have been prevalently used to represent the structural information, which raises the graph anomaly detection problem - identifying anomalous graph objects (i.e., nodes, edges and sub-graphs) in a single graph, or anomalous graphs in a database/set of graphs. However, conventional anomaly detection techniques cannot tackle this problem well because of the complexity of graph data. For the advent of deep learning, graph anomaly detection with deep learning has received a growing attention recently. In this survey, we aim to provide a systematic and comprehensive review of the contemporary deep learning techniques for graph anomaly detection. We compile open-sourced implementations, public datasets, and commonly-used evaluation metrics to provide affluent resources for future studies. More importantly, we highlight twelve extensive future research directions according to our survey results covering unsolved and emerging research problems and real-world applications. With this survey, our goal is to create a "one-stop-shop" that provides a unified understanding of the problem categories and existing approaches, publicly available hands-on resources, and high-impact open challenges for graph anomaly detection using deep learning.

==> tb2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Anomalous node Detection Table %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]
\centering
\footnotesize
\renewcommand\arraystretch{1}
\setlength{\tabcolsep}{2.8mm}
\caption{Summary of Anomalous Node Detection Techniques.}
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{m{2.1cm}<{\centering}|m{2.3cm}<{\centering}|m{1.1cm}<{\centering}|m{4cm}<{\centering}|m{1.8cm}<{\centering}|m{2.9cm}<{\centering}}
\toprule[1 pt]
\textbf{Graph Type} & \textbf{Approach} & \textbf{Category} & \textbf{Objective Function} & \textbf{Measurement} & \textbf{Outputs}  \\ 
\midrule[1 pt]
\multirow{3}{*}{\shortstack{Static Graph - \\ Plain}} & ~\cite{hu2016embedding} & NR & $\mathop{\sum}\limits_{(i,j)\in E} \|\mathbf{Z_{i}} - \mathbf{Z_{j}}\|^{2} + \alpha \mathop{\sum}\limits_{(i,j)\notin E}(\|\mathbf{Z_{i}} - \mathbf{Z_{j}}\| -1)^{2}$  & Anomaly Score  & $ \mathop{\sum}\limits_{k=1}^{d}\frac{y_{i}^{k}}{y_{i}^{*}}$ \\ \cline{2-6}
& DCI~\cite{wang2021decoupling} & NR &$\frac{1}{K}\mathop{\sum}\limits_{k=1}^K\mathcal{L}_{DCI}^{k}$ & Anomaly Prediction & Predicted Label \\\cline{2-6}

&NAC~\cite{morales2021selective} & RL & Cumulative reward  & -  & Anomalies \\ 


\midrule[1 pt]

\multirow{24}{*}{\shortstack{Static Graph - \\ Attributed}} &ALAD~\cite{liu2017accelerated} & Non-DP & $\min\limits_{W,H} \|A-WW^{T}\|_{F}^{2} + \alpha \|X-WH\|_{F}^{2} + \gamma (\|W\|_{F}^{2} + \|H\|_{F}^{2})$  & Anomaly Score & $\frac{\mathbf{W}_{n,c}}{\sum_{c}\mathbf{W}_{n,c}} cos(\mathbf{A}_{n*}, \mathbf{H}_{c*})$ \\   \cline{2-6}

&Radar~\cite{li2017radar} & Non-DP & $\min\limits_{W,R}\|X - W^{T} X - R\|_{F}^{2}+ \alpha \|W\|_{2,1} +\beta \|R\|_{2,1} +\gamma tr(R^{T}LR)$  & Residual Analysis & Residual Value \\  \cline{2-6}

&ANOMALOUS~\cite{peng2018anomalous} & Non-DP & $\min\limits_{W,\tilde{R}}||X - XWX - \tilde{R}||_{F}^{2} + \alpha ||W||_{2,1} + \beta ||W^{T}||_{2,1} +  \gamma ||\tilde{R}^{T}||_{2,1} + \varphi tr(\tilde{R}L\tilde{R}^{T})$ & Residual Analysis & Residual Value   \\  \cline{2-6}

&SGASD~\cite{wu2017adaptive} & Non-DP & $\min\limits_{\mathbf{w,c}}\frac{1}{2}\sum_{i=1}^{m}\mathbf{c_{i}}(V_{i,*}\mathbf{w} - y_i)^2 + \frac{\lambda_{1}}{2}||\mathbf{w}||_{2}^{2} + \lambda_{2} \sum_{i=0}^{d}\sum_{j=1}^{n_{i}}||\mathbf{c}_{G_{j}^{i}}||_{2}$  & Anomaly Prediction & Predicted Label \\  \cline{2-6}

&DONE~\cite{bandyopadhyay2020outlier} & DNN & $\alpha_{1}\mathcal{L}_{str}^{Recs} + \alpha_{2}\mathcal{L}_{attr}^{Recs} + \alpha_{3}\mathcal{L}_{str}^{Hom} + \alpha_{4}\mathcal{L}_{attr}^{Hom} + \alpha_{5}\mathcal{L}^{Com}$  & Anomaly Scores & $o_{i}^{s},o_{i}^{a},o_{i}^{com}$   \\  \cline{2-6}

&DOMINANT~\cite{ding2019deep} & GCN & $(1-\alpha)\mathcal{R}_{S} + \alpha \mathcal{R}_{A}$  & Anomaly Score & $(1-\alpha)||a_i - \hat{a}_i||_{2} + \alpha||x_i - \hat{x}_i||_{2}$ \\  \cline{2-6}

&ALARM~\cite{peng2020deep} & GCN & $\sum_{i=1}^n \sum_{j=1}^n - [\gamma A_{ij}\log\hat{A}_{ij} + (1-A_{ij})\log(1-\hat{A}_{ij})]$ & Anomaly Score & $(1-\alpha)||a_i - \hat{a}_i||^2_{2} + \alpha||x_i - \hat{x}_i||^2_{2}$  \\  \cline{2-6}

&SpecAE~\cite{li2019specae} & GCN & $\mathbb{E}[dis(X,\hat{X})] + \mathbb{E}[dis(X,\tilde{X})] + \lambda_{1}\mathbb{E}(E(Z)) + \lambda_{2}KL$ & Density Estimation & Anomalousness Rank  \\  \cline{2-6}

&Fdgars~\cite{wang2019fdgars} & GCN & $\mathcal{L}_{GCN}$ & Anomaly Prediction & Predicted Label  \\  \cline{2-6}

&GraphRfi~\cite{GraphRfi} & GCN & $\mathcal{L}_{rating} + \lambda \mathcal{L}_{fraudster}$ & Anomaly Prediction & Predicted Label  \\  \cline{2-6}

& ResGCN~\cite{pei2021resgcn} & GCN & $(1-\alpha)||A - \hat{A}||^2_{F} + \alpha||X - \hat{X} - \lambda R||^2_{F}$ & Anomaly Score & $||R_{i,:}||_{2}$  \\  \cline{2-6}

&GraphUCB~\cite{ding2019interactive} & RL & Expert Judgment  & - & Anomalies \\  \cline{2-6}

&AnomalyDAE~\cite{fan2020anomalydae} & GAT & $\alpha ||(A - \hat{A})\odot \bm{\theta}||_{F}^{2} + (1-\alpha)||(X - \hat{X})\odot \bm{\eta}||_{F}^{2}$ & Reconstruction Loss & Anomalousness Rank \\  \cline{2-6}

&SemiGNN~\cite{SemiGNN} & GAT & $\alpha \mathcal{L}_{sup} + (1- \alpha) \mathcal{L}_{unsup} + \lambda \mathcal{L}_{reg}$ & Anomaly Prediction & Predicted Label \\  \cline{2-6}

&AEGIS~\cite{ding2020inductive} & GAN & $\mathcal{L}_{AE} + \mathcal{L}_{GAN}$ & Anomaly Score & $1 - D(z_i)$ \\  \cline{2-6}

&REMAD~\cite{zhang2019robust} & NR & $\mathcal{L}_{res} + \beta\| R^{T}\|_{2,1}$  & Residual Analysis & Residual Value \\  \cline{2-6}

&CARE-GNN~\cite{CARE-GNN} & NR & $\mathcal{L}_{GNN} + \lambda_{1}\mathcal{L}_{Simi}^{(1)} + \lambda_{2}\mathcal{L}_{reg}$  & Anomaly Prediction & Predicted Label \\  \cline{2-6}

&SEANO~\cite{liang2018semi} & NR & $-\sum_{i \in V_{L}} \log p(y_{i}|\mathbf{x}_{i},\Bar{\mathbf{x}}_{N_{i}}) - \sum_{i \in V}\sum_{v\prime \in C_i} \log p(v\prime|\mathbf{x}_{i},\Bar{\mathbf{x}}_{N_{i}})$  & Anomaly Score & Discriminator's Output \\ \cline{2-6}

&OCGNN~\cite{wang2020ocgnn} & NR & $\frac{1}{\beta K}\sum\limits_{v_{i}\in\mathbf{V}_{tr}}[||g(X,A;\mathcal{W})_{v_i}-c||^2 -r^2]^{+}+ r^2 +\frac{\lambda}{2}\sum\limits_{l=1}^{L}||W^{(l)}||^2$  & Location in Embedding Space & Distance to Hypersphere Center \\ \cline{2-6}

&GAL~\cite{GAL} & NR &  $\max\{0,\max\limits_{y_{v^{\prime}} \neq y_{u}}g(u,v^\prime) - \min\limits_{y_{v} = y_{u}}g(u,v) + \Delta_{y_u}\}$  & Anomaly Prediction & Predicted Label \\ \cline{2-6}
 
&CoLA~\cite{liu2021anomaly}& NR & $-\sum\limits_{i=1}^{N}y_{i}\log(CLM(v_i,\mathcal{G}_{i})) + (1-y_i)\log(1-CLM(v_i,\mathcal{G}_{i}))$  & Anomaly Score & $\frac{\sum\limits_{r=1}^{R}(s_{i,r}^{(-)}-s_{i,r}^{(+)})}{R}$ \\ \cline{2-6}

&COMMANDER~\cite{ding2021cross} & NR & $-\mathcal{L}_{D} + \mathcal{L}_{C} + \mathcal{L}_{R}$  & Anomaly Score & $\bar{y_i}||\mathbf{\tilde{x}_i} - \mathbf{x}_i||_2^2$ \\ \cline{2-6}

&FRAUDRE~\cite{zhangge1}& NR & $\sum\limits_{i=1}^{n}f^{*}(y_i,\mathbf{h}_{i}^{(final)}\mathbf{W}_2)$  & Anomaly Prediction & Predicted Label \\ \cline{2-6}

&Meta-GDN~\cite{ding2021few} & NR & $(1-y_i)\cdot|dev(v_i)| + y_i\cdot\max(0,dev(v_i))$  & Anomaly Score & $\mathbf{u}_{s}^{T}\mathbf{o}_{i} + b_s$ \\ 

\midrule[1 pt]

Dynamic Graph - Plain & NetWalk~\cite{yu2018netwalk} & DNN & $\gamma\mathcal{L}_{AE} + \mathcal{L}_{Clique} + \lambda\|W\|_{F}^{2} + \beta KL$ & Anomaly Score & Nearest Distance to Cluster Centers \\ [2ex]
\midrule[1 pt]

\multirow{2}{*}{\shortstack{Dynamic Graph - \\ Attributed}} &MTHL~\cite{teng2017anomaly} & Non-DP & $\mathop{min}_{\mathcal{P}}f(\mathcal{P})$  & Anomaly Score & Distance to Hypersphere Centroid \\  \cline{2-6}
&OCAN~\cite{zheng2019one} & GAN & $\mathcal{L}_{LSTM-AE} + \mathcal{L}_{GAN}$  & Anomaly Score & Discriminator's Output  \\

\bottomrule[1 pt]
\multicolumn{6}{l}{* Non-DP: Non-Deep Learning Techniques, DNN: Deep NN Based Techniques, GCN: GCN Based Techniques, RL: Reinforcement Learning Based Techniques.} \\
\multicolumn{6}{l}{* GAT: GAT Based Techniques, NR: Network Representation Based Techniques, GAN: Generative Adversarial Network Based Techniques.}
\end{tabular}
}
\label{table:ANOSND}
\end{table*}

==> tb3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Anomalous edge and subgraph detection Table %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!h]
\centering 
\footnotesize
\renewcommand\arraystretch{1}
\setlength{\tabcolsep}{2.8mm}
\caption{Summary of Anomalous Edge, Sub-graph and Graph Detection Techniques.} 
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{m{2.1cm}<{\centering}|m{2.3cm}<{\centering}|m{1.1cm}<{\centering}|m{4cm}<{\centering}|m{1.8cm}<{\centering}|m{2.9cm}<{\centering}}
\toprule[1 pt]
\textbf{Graph Type} & \textbf{Approach} & \textbf{Category} & \textbf{Objective Function} & \textbf{Measurement} & \textbf{Outputs}  \\ 
\midrule[1 pt]
\multicolumn{6}{c}{Anomalous Edge Detection Techniques} \\
\midrule[1 pt]
\multirow{2}{*}{\shortstack{Static Graph - \\ Plain}} &UGED~\cite{DBLP:conf/ijcnn/Ouyang0020} & DNN & $\text{cross-entropy}(f(u,N(u)), v)$  & Anomaly Score  & $\text{mean}(1-P(v|u,N(u)), 1-P(u|v,N(v)))$ \\  \cline{2-6}
&AANE~\cite{AANE} & GCN & $\mathcal{L} = \mathcal{L}_{afl} + \gamma\mathcal{L}_{aal}$  & Anomaly Ranking  & Edge Existing Probability \\ 
\midrule[1 pt]

Static Graph - Attributed &eFraudCom~\cite{zhangge2} & NR & $\mathcal{L}_{MAIN} - \lambda\mathcal{L}_{MI}$ & Anomaly Prediction & Predicted Label \\ 

\midrule[1 pt]

Dynamic Graph - Plain & NetWalk~\cite{yu2018netwalk} & NR & $\mathcal{L}_{AE} + \mathcal{L}_{Clique} + \|W\|_{F}^{2} + KL $  & Anomaly Score & Nearest Distance to Cluster Centers \\
\midrule[1 pt]

Dynamic Graph - Attributed & AddGraph~\cite{zheng2019addgraph} & GCN & $\text{min} \sum_{{e\in \varepsilon^{t}}}\sum_{{e^{\prime}\notin \varepsilon^{t}}} \text{max}\{0, \gamma + f(i,j,w) - f(i^{\prime},j^{\prime},w)\} + \lambda\mathcal{L}_{reg}$  & Anomaly Score & $f(i,j,w) = w\cdot\sigma(\beta\cdot (||\mathbf{a} \odot \mathbf{h}_{i} + \mathbf{b} \odot \mathbf{h}_{j}||^{2}_{2} - \mu))$ \\ 

\midrule[1 pt]
\midrule[1 pt]
\multicolumn{6}{c}{Anomalous Sub-graph Detection Techniques} \\
\midrule[1 pt]
\multirow{2}{*}{\shortstack{Static Graph - \\ Plain}} &DeepFD~\cite{wang2018deep} & NR & $\mathcal{L}_{recon} +\alpha \mathcal{L}_{sim} + \gamma \mathcal{L}_{reg}$& Density-based Method (DBSCAN)  & Dense sub-graphs \\   \cline{2-6}

&FraudNE~\cite{FraudNE} & NR & $\mathcal{L}_{res}^{source} + \mathcal{L}_{res}^{sink} + \alpha \mathcal{L}_{share} + \eta \mathcal{L}_{reg}$  & Density-based Method (DBSCAN)  & Dense sub-graphs \\

\midrule[1 pt]
\midrule[1 pt]

\multicolumn{6}{c}{Anomalous Graph Detection Techniques} \\
\midrule[1 pt]
\multirow{2}{*}{\shortstack{Graph Database - \\ Attributed}}&UPFD~\cite{dou2021user} & NR & $ -(y\log(p) + (1-y)\log(1-p))$ & Anomaly Prediction & Predicted Label \\ \cline{2-6}
%Graph Database - Attributed 
& OCGIN~\cite{zhao2020using} & GNN & $ \min\limits_{W}\frac{1}{N}\sum\limits_{i=1}^{N}||GIN(G_i,W)-c||^2 + \frac{\lambda}{2}\sum\limits_{l=1}^{L}||W^l||^2_{F}$ & Location in Embedding Space & Distance to Hypersphere Center \\
\midrule[1 pt]

\multirow{2}{*}{\shortstack{Dynamic Graph - \\ Plain}} & DeepSphere~\cite{teng2018deep} & DNN & $\mathcal{L} = \mathcal{L}_{h} + \lambda\mathcal{L}_{res}$ & Location in Embedding Space  & Anomalous Label  \\ \cline{2-6}
& GLAD-PAW~\cite{wan2021glad} & GNN & $\text{cross-entropy}(\mathbf{y},\mathbf{\hat{y}})$ & Anomaly Prediction  & Predicted Label  \\ 

\bottomrule[1 pt]
\multicolumn{6}{l}{* DNN: Deep NN Based techniques, GCN: GCN Based Techniques, NR: Network Representation Based Techniques.}\\
\multicolumn{6}{l}{* GNN: Graph Neural Network Based Techniques.}
\end{tabular}
\label{tb:edgeandsubgraph}
}
\end{table*}

==> tb4.tex <==
\begin{table*}[!t]
\centering 
\footnotesize
\renewcommand\arraystretch{1}
\setlength{\tabcolsep}{2.8mm}
\caption{Published Algorithms and Models} 
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{c|c|c|c|l}
\toprule[1 pt]
\textbf{Model} & \textbf{Language} & \textbf{Platform} &  \textbf{Graph} & \textbf{Code Repository} \\ 
\midrule[1 pt]


AnomalyDAE~\cite{fan2020anomalydae}  & Python & Tensorflow   & Static Attributed Graph & https://github.com/haoyfan/AnomalyDAE   \\ \hline

MADAN~\cite{gutierrez2020multi}    & Python & -   & Static Attributed Graph & https://github.com/leoguti85/MADAN  \\ \hline

PAICAN~\cite{bojchevski2018bayesian}  & Python & Tensorflow  & Static Attributed Graph & http://www.kdd.in.tum.de/PAICAN/   \\ \hline

ONE~\cite{bandyopadhyay2019outlier} & Python & -  & Static Attributed Graph & https://github.com/sambaranban/ONE   \\ \hline

DONE\&AdONE~\cite{bandyopadhyay2020outlier}  & Python & Tensorflow    & Static Attributed Graph & https://bit.ly/35A2xHs \\ \hline

SLICENDICE~\cite{nilforoshan2019slicendice}  & Python & -  & Static Attributed Graph & http://github.com/hamedn/SliceNDice/ \\ \hline

FRAUDRE~\cite{zhangge1}  & Python & Pytorch  & Static Attributed Graph & https://github.com/FraudDetection/FRAUDRE \\ \hline

SemiGNN~\cite{SemiGNN}  & Python & Tensorflow  & Static Attributed Graph & https://github.com/safe-graph/DGFraud \\ \hline

CARE-GNN~\cite{CARE-GNN}  & Python & Pytorch & Static Attributed Graph & https://github.com/YingtongDou/CARE-GNN \\ \hline

GraphConsis~\cite{GraphConsis}  & Python & Tensorflow  & Static Attributed Graph & https://github.com/safe-graph/DGFraud \\ \hline

GLOD~\cite{zhao2020using}  & Python & Pytorch  & Static Attributed Graph & https://github.com/LingxiaoShawn/GLOD-Issues \\ \hline

OCAN~\cite{zheng2019one} & Python & Tensorflow  & Static Graph &https://github.com/PanpanZheng/OCAN \\ \hline

DeFrauder~\cite{DBLP:conf/ijcai/DhawanGK019} & Python & -  & Static Graph & https://github.com/LCS2-IIITD/DeFrauder \\ \hline

GCAN~\cite{lu2020gcan}  & Python & Keras & Heterogeneous Graph & https://github.com/l852888/GCAN \\ \hline

HGATRD~\cite{huang2020heterogeneous} & Python & Pytorch   & Heterogeneous Graph & https://github.com/201518018629031/HGATRD  \\\hline

GLAN~\cite{yuan2019jointly}  & Python & Pytorch  & Heterogeneous Graph & https://github.com/chunyuanY/RumorDetection \\ \hline

GEM~\cite{liu2018heterogeneous} & Python & -  & Heterogeneous Graph & https://github.com/safe-graph/DGFraud/tree/master/algorithms/GEM \\ \hline

eFraudCom~\cite{zhangge2} & Python & Pytorch & Heterogeneous Graph & https://github.com/GeZhangMQ/eFraudCom \\ \hline

DeepFD~\cite{wang2018deep} & Python & Pytorch  & Bipartite Graph & https://github.com/JiaWu-Repository/DeepFD-pyTorch \\ \hline

ANOMRANK~\cite{yoon2019fast} & C++ & - & Dynamic Graph & https://github.com/minjiyoon/anomrank \\ \hline

MIDAS~\cite{DBLP:conf/aaai/0001HYSF20} & C++ & - & Dynamic Graph & https://github.com/Stream-AD/MIDAS \\ \hline

Sedanspot~\cite{eswaran2018sedanspot}    & C++ &  -   & Dynamic Graph & https://www.github.com/dhivyaeswaran/sedanspot \\ \hline

F-FADE~\cite{chang2021f} & Python & Pytorch  & Dynamic Graph & http://snap.stanford.edu/f-fade/ \\ \hline

DeepSphere~\cite{teng2018deep}  & Python & Tensorflow   & Dynamic Graph & https://github.com/picsolab/DeepSphere   \\ \hline

Changedar~\cite{hooi2018changedar}  & Matlab & -   & Dynamic Graph & https://bhooi.github.io/changedar/  \\\hline

UPFD~\cite{dou2021user} & Python & Pytorch  & Graph Database & https://github.com/safe-graph/GNN-FakeNews \\ \hline

OCGIN~\cite{zhao2020using} & Python & Pytorch  & Graph Database & https://github.com/LingxiaoShawn/GLOD-Issues \\ \hline

DAGMM~\cite{zong2018deep} & Python & Pytorch  &  Non Graph & https://github.com/danieltan07/dagmm \\ \hline

DevNet~\cite{pang2019deep} & Python & Tensorflow  & Non Graph &https://github.com/GuansongPang/deviation-network \\ \hline

RDA~\cite{zhou2017anomaly} & Python & Tensorflow & Non Graph &https://github.com/zc8340311/RobustAutoencoder \\ \hline

GAD~\cite{GAD} & Python & Tensorflow  & Non Graph &https://github.com/raghavchalapathy/gad \\ \hline

Deep SAD~\cite{ruff2019deep} &Python & Pytorch  & Non Graph & https://github.com/lukasruff/Deep-SAD-PyTorch \\ \hline

DATE~\cite{10.1145/3394486.3403339} &Python & Pytorch  &Non Graph & https://github.com/Roytsai27/Dual-Attentive-Tree-aware-Embedding \\ \hline

STS-NN~\cite{STS-NN} & Python & Pytorch  & Non Graph & https://github.com/JiaWu-Repository/STS-NN \\
\bottomrule[1 pt]
\multicolumn{5}{l}{* -: No Dedicated Platforms.}
\end{tabular}
\label{tb:publishedalgs}
}
\end{table*}
